Mitigating Homophily Disparity in Graph Anomaly Detection: A Scalable and Adaptive Approach

Graph anomaly detection (GAD) aims to identify nodes that deviate from normal patterns in structure or features. While recent GNN-based approaches have advanced this task, they struggle with two major challenges: 1) homophily disparity, where nodes exhibit varying homophily at both class and node levels; and 2) limited scalability, as many methods rely on costly whole-graph operations. To address them, we propose SAGAD, a Scalable and Adaptive framework for GAD. SAGAD precomputes multi-hop embeddings and applies reparameterized Chebyshev filters to extract low- and high-frequency information, enabling efficient training and capturing both homophilic and heterophilic patterns. To mitigate node-level homophily disparity, we introduce an Anomaly Context-Aware Adaptive Fusion, which adaptively fuses low- and high-pass embeddings using fusion coefficients conditioned on Rayleigh Quotient-guided anomalous subgraph structures for each node. To alleviate class-level disparity, we design a Frequency Preference Guidance Loss, which encourages anomalies to preserve more high-frequency information than normal nodes. SAGAD supports mini-batch training, achieves linear time and space complexity, and drastically reduces memory usage on large-scale graphs. Theoretically, SAGAD ensures asymptotic linear separability between normal and abnormal nodes under mild conditions. Extensive experiments on 10 benchmarks confirm SAGAD's superior accuracy and scalability over state-of-the-art methods.

==> tables/ablation_auroc.tex <==
\begin{table*}[t]
  \centering
  {\caption{Ablation study on each component of our SAGAD in terms of AUROC.}
  \label{Tab: Ablation Study AUROC}}
  % \setlength{\tabcolsep}{3pt}
  % \resizebox{1.\textwidth}{!}{
  \begin{tabular}{ccccc|ccccccc}
  \toprule
    $\boldsymbol{Z}_L$ & $\boldsymbol{Z}_H$ & $\mathcal{G}^{RQ}$ & $\mathcal{L}_{fpg}$ & Fusion & Reddit & Amazon & Yelp. & T-Fin. & Ellip. & Tolo. & DGraph. \\ \midrule
    \ding{51} & \ding{51} & \ding{51} & \ding{51} & Eq. (7) & \textbf{66.5±3.0} & \textbf{94.5±2.1} & \textbf{68.8±2.5} & \textbf{94.4±0.4} & \textbf{90.9±0.9} & \textbf{73.6±0.8} & \textbf{70.8±1.9} \\
    \ding{51} & \ding{51} & \ding{51} & \ding{55} & Eq. (7) & 63.9±3.6 & 94.3±1.9 & 68.1±2.5 & 93.2±2.1 & 90.5±1.1 & 69.1±1.8 & 69.6±1.3 \\
    \ding{51} & \ding{51} & \ding{66} & \ding{51} & Eq. (7) & 65.6±2.9 & 93.8±2.0 & 63.9±4.3 & 93.2±1.3 & 90.1±1.2 & 68.2±1.7 & 69.0±1.3 \\
    \ding{51} & \ding{51} & \ding{55} & \ding{51} & Eq. (7) & 63.8±3.7 & 93.9±2.1 & 63.8±4.3 & 93.3±1.3 & 90.2±1.2 & 68.8±1.2 & 69.1±1.5 \\
    \ding{51} & \ding{51} & \ding{55} & \ding{55} & Mean & 66.0±2.4 & 93.9±2.0 & 64.1±4.8 & 88.2±1.3 & 90.4±0.7 & 68.3±1.4 & 68.8±1.4 \\
    \ding{51} & \ding{51} & \ding{55} & \ding{55} & Concat & 61.3±5.0 & 93.6±2.7 & 64.0±4.1 & 93.6±0.9 & 89.9±1.3 & 70.2±1.8 & 70.0±1.9 \\
    \ding{51} & \ding{51} & \ding{55} & \ding{55} & Atten. & 63.2±3.5 & 94.4±2.3 & 63.7±4.4 & 91.8±1.7 & 85.7±1.8 & 69.7±1.9 & 70.0±2.0 \\
    \ding{51} & \ding{55} & \ding{55} & \ding{55} & - & 58.0±6.3 & 81.8±0.7 & 52.8±1.8 & 92.4±0.6 & 89.1±1.2 & 71.0±1.1 & 65.1±2.1 \\
    \ding{55} & \ding{51} & \ding{55} & \ding{55} & - & 60.3±2.9 & 93.1±2.1 & 63.0±4.0 & 78.0±2.9 & 85.4±1.1 & 65.9±2.6 & 69.4±1.0 \\
  \bottomrule
  \end{tabular}
  % }
\end{table*}


==> tables/ablation_reck.tex <==
\begin{table*}[t]
  {\caption{Ablation study on each component of our SAGAD in terms of Rec@K.}
  \label{Tab: Ablation Study RecK}}
  \centering
  % \setlength{\tabcolsep}{3pt}
  % \resizebox{1.\textwidth}{!}{
  \begin{tabular}{ccccc|ccccccc}
  \toprule
    $\boldsymbol{Z}_L$ & $\boldsymbol{Z}_H$ & $\mathcal{G}^{RQ}$ & $\mathcal{L}_{fpg}$ & Fusion & Reddit & Amazon & Yelp. & T-Fin. & Ellip. & Tolo. & DGraph. \\ \midrule
    \ding{51} & \ding{51} & \ding{51} & \ding{51} & Eq. (7) & \textbf{8.6±1.7} & \textbf{80.8±1.3} & \textbf{31.5±2.7} & \textbf{78.3±1.3} & \textbf{59.4±2.7} & \textbf{40.2±1.9} & \textbf{3.6±1.0} \\
    \ding{51} & \ding{51} & \ding{51} & \ding{55} & Eq. (7) & 7.9±1.6 & 79.3±2.4 & 30.4±2.2 & 74.0±5.1 & 59.0±3.5 & 37.0±2.5 & 2.8±0.7 \\
    \ding{51} & \ding{51} & \ding{66} & \ding{51} & Eq. (7) & 8.0±1.9 & 78.5±2.0 & 25.8±3.5 & 73.5±3.7 & 57.7±3.6 & 35.5±1.4 & 2.4±0.8 \\
    \ding{51} & \ding{51} & \ding{55} & \ding{51} & Eq. (7) & 7.6±1.6 & 78.8±1.6 & 25.7±3.4 & 74.5±3.6 & 57.9±3.8 & 35.5±1.9 & 2.6±0.7 \\
    \ding{51} & \ding{51} & \ding{55} & \ding{55} & Mean & 8.3±1.6 & 77.7±2.6 & 25.7±3.7 & 63.7±0.4 & 59.0±3.9 & 34.5±1.6 & 2.6±1.0 \\
    \ding{51} & \ding{51} & \ding{55} & \ding{55} & Concat & 6.7±2.0 & 75.6±6.9 & 26.3±3.8 & 74.7±2.8 & 56.9±4.3 & 38.4±2.8 & 3.1±1.0 \\
    \ding{51} & \ding{51} & \ding{55} & \ding{55} & Atten. & 6.1±2.4 & 78.5±1.9 & 25.9±3.7 & 68.9±4.0 & 42.7±7.8 & 36.5±2.5 & 2.8±1.1 \\
    \ding{51} & \ding{55} & \ding{55} & \ding{55} & - & 5.9±2.0 & 36.5±2.2 & 17.9±1.8 & 72.5±2.0 & 50.0±3.1 & 37.8±2.0 & 2.8±1.1 \\
    \ding{55} & \ding{51} & \ding{55} & \ding{55} & - & 7.5±1.8 & 76.8±2.9 & 25.1±3.5 & 28.2±4.6 & 46.6±3.5 & 32.1±3.4 & 2.1±0.3 \\
  \bottomrule
  \end{tabular}
  % }
\end{table*}

